Reverse Link Analysis for Full-Duplex Cellular Networks with Low Resolution ADC/DAC

In this work, we consider a full-duplex (FD) massive multiple-input multiple-output (MIMO) cellular network with low-resolution analog-to-digital converters (ADCs) and digital-to-analog converter (DACs). Our first contribution is to provide a unified framework for reverse link (uplink) analysis where matched filters are applied at the FD base stations (BSs) under channel hardening. Second, we derive the expressions of the signal-to-quantization-plus-interference-plus-noise ratio (SQINR) for general and special cases. Finally, we quantify effects of quantization error, pilot contamination, and full duplexing for a hexagonal cell lattice on spectral efficiency and cumulative distribution function (CDF) to show that FD outperforms half duplex (HD) in a wide variety of scenarios.

==> asymptotic.tex <==
\section{Asymptotic Analysis and Power Scaling Laws}
In the section, we investigate the effects of the number of quantization bits, the number of antennas at the BS, the number of users, the power budgets of the BS and each user on the spectral efficiency performance for reverse link. In the sequel, we carry out the analysis for the channel hardening case. 

\begin{lemma}\label{lemma2}
For a fixed power budget, fixed number of transmit antennas and full-resolution ($b \rightarrow \infty$, $\alpha_u = \alpha_d = 1$), the spectral efficiency converges to (\ref{uplinklemma2}).
\end{lemma}
\begin{figure*}
\begin{equation}\label{uplinklemma2}
\frac{\bar{\mathcal{I}}^\mathsf{MF}}{B} \rightarrow \log\left(1+ \frac{\frac{\left( \frac{P_k^u}{P_u}\mathsf{SNR}_k^u \right)^2N_a}{ 1+\frac{P^u_k}{P_u}\mathsf{SNR}_k^u + \sum_{\ell \in \mathcal{C}}\frac{P_{\ell,k}^u}{P_u}\mathsf{SNR}_{\ell,k}^u  } } { 1 + \sum_{\ell}\sum_{\text{k}=0}^{K_\ell^u-1} \frac{P_{\ell,\text{k}}^u}{P_u} \mathsf{SNR}_{\ell,\text{k}}^u  + N_a\frac{\sum_{\ell \in \mathcal{C}}\left( \frac{P_{\ell,k}^u}{P_u} \mathsf{SNR}_{\ell,k}^u \right)^2}{1 + \frac{P_k^u}{P_u}\mathsf{SNR}_k^u + \sum_{\ell \in \mathcal{C}}\frac{P_{\ell,k}}{P_u}\mathsf{SNR}_{\ell,k}^u} +N_a K^d\mathsf{INR}} \right)   
\end{equation}
\end{figure*}
\begin{lemma}\label{lemma3}
For a fixed number of antennas and fixed $b$, when $\mathsf{SNR}_k^u\rightarrow \infty$, the spectral efficiency converges to (\ref{uplinklemma3}). 
\end{lemma}
\begin{equation}\label{uplinklemma3}
\frac{\bar{\mathcal{I}}^\mathsf{MF}}{B} \rightarrow \log\left( 1 + \frac{N_a}{\alpha_u(2-\alpha_u)}  \right)
\end{equation}
\begin{lemma}\label{lemma4}
If the transmit powers of the BS and each user is scaled with the number of antennas $N_a$ i.e., $P = \frac{E}{N_a}$ where $E$ is fixed, as $N_a \rightarrow \infty$, the spectral efficiency converges to (\ref{uplinklemma4}).
\end{lemma}
\begin{equation}\label{uplinklemma4}
\frac{\bar{\mathcal{I}}^\mathsf{MF}}{B} \rightarrow \log\left(1 +\frac{\alpha_u \left(  \frac{E_k^u}{E_u} \mathsf{SNR}_k^u \right)^2}{1+\alpha_d\left( \alpha_uK^d + 1-\alpha_u \right)\mathsf{INR} }  \right)    
\end{equation}

\begin{lemma}\label{lemma5}
If the transmit power and the number of users per cell are fixed, as $N_a/K\rightarrow \infty$, the spectral efficiency converges to (\ref{uplinklemma5}). 
\end{lemma}
\begin{figure*}
\begin{equation}\label{uplinklemma5}
 \frac{\bar{\mathcal{I}}^\mathsf{MF}}{B} \rightarrow \log\left(1 + \frac{ \frac{\alpha_u \left( \frac{P_k^u}{P_u}\mathsf{SNR}_k^u \right)^2   }{1+\frac{P^u_k}{P_u}\mathsf{SNR}_k^u + \sum_{\ell \in \mathcal{C}}\frac{P_{\ell,k}^u}{P_u}\mathsf{SNR}_{\ell,k}^u }     }{      \alpha_u \frac{\sum_{\ell \in \mathcal{C}}\left( \frac{P_{\ell,k}}{P_u} \mathsf{SNR}_{\ell,k}^u \right)^2}{1 + \frac{P_k}{P_u}\mathsf{SNR}_k^u + \sum_{\ell \in \mathcal{C}}\frac{P_{\ell,k}}{P_u}\mathsf{SNR}_{\ell,k}^u} +\alpha_d\left(\alpha_uK^d + 1-\alpha_u \right) \mathsf{INR} }  \right)
\end{equation}
\end{figure*}






